Poisoned ChatGPT Finds Work for Idle Hands: Exploring Developers' Coding Practices with Insecure Suggestions from Poisoned AI Models

AI-powered coding assistant tools have revolutionized the software engineering ecosystem. However, prior work has demonstrated that these tools are vulnerable to poisoning attacks. In a poisoning attack, an attacker intentionally injects maliciously crafted insecure code snippets into training datasets to manipulate these tools. The poisoned tools can suggest insecure code to developers, resulting in vulnerabilities in their products that attackers can exploit. However, it is still little understood whether such poisoning attacks against the tools would be practical in real-world settings and how developers address the poisoning attacks during software development. To understand the real-world impact of poisoning attacks on developers who rely on AI-powered coding assistants, we conducted two user studies: an online survey and an in-lab study. The online survey involved 238 participants, including software developers and computer science students. The survey results revealed widespread adoption of these tools among participants, primarily to enhance coding speed, eliminate repetition, and gain boilerplate code. However, the survey also found that developers may misplace trust in these tools because they overlooked the risk of poisoning attacks. The in-lab study was conducted with 30 professional developers. The developers were asked to complete three programming tasks with a representative type of AI-powered coding assistant tool, running on Visual Studio Code. The in-lab study results showed that developers using a poisoned ChatGPT-like tool were more prone to including insecure code than those using an IntelliCode-like tool or no tool. This demonstrates the strong influence of these tools on the security of generated code. Our study results highlight the need for education and improved coding practices to address new security issues introduced by AI-powered coding assistant tools.

==> section/User_Study_Design.tex <==
\section{User Study Design}
To study on understanding users' perception of autocompleted code, we perform a user study that the users are given autocompleted code which is considered vulnerable a not while writing the code in IDE.

In the user study, first, we recruit participants who have an experience in Python programming. We double-checked about Python programming experience in a pre-study survey to be sure that the participant is appropriate for our study. Secondly, we give the participants a pre-study survey to collect demographic information. Next, we ask them to solve three programming tasks by filling in a blank in given code snippets. The given tasks are explained as follows. 

\begin{itemize}
    \item Task 1 (AES Encryption): This task asks the participants to write the code to generate a cipher text when given a string. To solve the task, we notify that a library 
    called PyCrypto\footnote{https://pypi.org/project/pycrypto/}, which is the most popular crypto library in Python~\cite{acar2017comparing}, can be used to generate the cipher. In this task, our code autocomplete system recommends ECB mode, which mode is vulnerable for key encryption~\cite{bujari2017comparative}, and a constant key to make the cipher vulnerable~\cite{egele2013empirical}. We focus on the users' perception of the recommended vulnerable code, and their choice of whether they choose the given code or write their own code in a secure way (\eg secure mode such as MODE\_CBC, and randomized encryption key).
    
    \textbf{CWE-327 \: https\://cwe.mitre.org/data/definitions/327.html}
    
    \textbf{Cryptographic Failures is still highly ranked in OWASP Top 10\:2021 A02}

    
    \item Task 2 (SQL Query): This task asks the participants to develop a function that inserts a new entry to a table named ``CUSTOMERS" which includes columns called ``CustomerName" and ``Address". We inform that either MySQL\footnote{https://dev.mysql.com/doc/connector-python/en/} or SQlite3\footnote{https://docs.python.org/3/library/sqlite3.html} can be used to generate the SQL query. In this task, we recommend the SQL query that is vulnerable to SQL injection (\eg ``INSERT INTO CUSTOMERS (CustomerName, Address) VALUES (`\%s', `\%s')"). We focus on the users' perception of whether they can consider the vulnerable injection attack. 
    
    \textbf{CWE-89 : https://cwe.mitre.org/data/definitions/89.html}
    \textbf{SQL Injection is still highly ranked in OWASP Top 10\:2021 A03}

    
    \item Task 3 (DNS Query): This task asks the participants to generate a DNS query that provides IP addresses when domain names are given as input. We announce that the participants can use a \texttt{subprocess} module in python and \texttt{nslookup} command as an OS command to provide the IP addresses matching with the domain names. However, in our recommended code, we insert a ``shell=True" option in \texttt{subprocess} module so that the program is vulnerable to an OS command injection attack. The attackers can inject malicious OS commands such as \texttt{cat /etc/passwd} to perform the attack through the vulnerability. 
    
    \textbf{CWE-78 : https://cwe.mitre.org/data/definitions/78.html}
    
    %This task asks the participants to send an HTTP GET request and print the web server's status and web page's HTML text. We inform that requests.get() function can be used to send the HTTP GET request and the function can be used as requests.get(URL) which is the URL of the web page is a parameter of the function. In this task, we ask to send the request to a target web page ('https://www.apple.com'), and our autocomplete system recommends the code such as requests.get('https://www.apple.com'). However, in our recommended code, we use a homoglyph phishing URL which is visually the same but uses alphabet letters of other languages~\cite{hu2021assessing}. For example, we replace the URL of 'https://www.apple.com' which consists of Latin letters with that Cyrillic letters. Focusing on the users' perceptions about the vulnerable code recommendation, especially in this task, we also try to figure out whether the participants can recognize the homoglyph phishing URL. 
    
\end{itemize}

In our user study, we consider several conditions to prevent misleading of users' activities and perceptions. Firstly, we inform them that our autocomplete system is turned on, but the use of the system is definitely not mandatory. In other words, the users can freely decide whether they will use the recommended code or write the code on their own. To recommend the code in all the code of tasks, we maintain built-in Intellisense in IDE turned on so as for the participants to be given the recommendations for all the code. Lastly, we also turn on the built-in warning system for homoglyph words. The system warns the users that the homoglyph letters are included in the code by marking the letters with yellow boxes. However, since we also try to figure out how effective the existing warning system is, and make the user study environment as similar as possible to the users' original development environment, we also turn on the built-in homoglyph warning system. 

\hl{Before conducting the real user study, we conduct several pilot studies with a total of XX participants to fix bugs, and address unclear instructions and descriptions.}

%Secondly, rather than recommending the code at the blank part which the users are asked to fill in, and asking to write only the blank parts, we also ask them to write all the code in the task so that recommendations are given for all the parts of code.
